Communication-Efficient Device Scheduling for Federated Learning Using Lyapunov Optimization

Federated learning (FL) is a useful tool that enables the training of machine learning models over distributed data without having to collect data centrally. When deploying FL in constrained wireless environments, however, intermittent connectivity of devices, heterogeneous connection quality, and non-i.i.d. data can severely slow convergence. In this paper, we consider FL with arbitrary device participation probabilities for each round and show that by weighing each device's update by the reciprocal of their per-round participation probability, we can guarantee convergence to a stationary point. Our bound applies to non-convex loss functions and non-i.i.d. datasets and recovers state-of-the-art convergence rates for both full and uniform partial participation, including linear speedup, with only a single-sided learning rate. Then, using the derived convergence bound, we develop a new online client selection and power allocation algorithm that utilizes the Lyapunov drift-plus-penalty framework to opportunistically minimize a function of the convergence bound and the average communication time under a transmit power constraint. We use optimization over manifold techniques to obtain a solution to the minimization problem. Thanks to the Lyapunov framework, one key feature of the algorithm is that knowledge of the channel distribution is not required and only the instantaneous channel state information needs to be known. Using the CIFAR-10 dataset with varying levels of data heterogeneity, we show through simulations that the communication time can be significantly decreased using our algorithm compared to uniformly random participation, especially for heterogeneous channel conditions.

==> Sampling.tex <==
\section{Optimizing the Number of Sampling with Replacement Draws $m$}\label{sec:opt_m}
\noindent \jake{Note: Will probably remove this section.
The goal of this section is to explore the optimal number of sampling with replacement draws per round given different distributions of communication and computation time.
The value of this section is dependent on whether the metric of maximizing the number of samples seen/learned from per second is a convincing proxy for speeding up convergence in terms of wall-clock time.
The results do show that an optimal number of draws exist just like in our experiments, however, the numbers don't match.
The plot of the results in Figure \ref{fig:opt_m} is interesting, but since it doesn't quite match up with experimental results, its impact isn't as strong as I hoped.
Also, note that there are some minor errors in the analysis shown below that I've since fixed, but haven't updated here yet (besides in the plot).
I will obviously update it if y'all think this section is worth keeping even in a compressed form.
Let me know your thoughts!}

Up to this point, we have treated $m$, the number of sampling with replacement draws per round, as a given, user-defined hyperparameter.
Choosing the best value for $m$, however, is not a straightforward task.
In fact, it is an open problem even in the standard uniform sampling case.
In this section, we will discuss how it is closely related to choosing the optimal batch size in SGD which is also not mathematically understood and is typically fine-tuned via trial and error.
As opposed to centralized training, when performing FL over wireless channels with limited resources, systems typically cannot afford to train multiple models with varying hyperparameters to find the best results.
Thus, it is imperative to develop a strategy to determine a viable $m$ before run-time.
While we focus on mathematical analysis here, we also explore this empirically in our experiments in Section \ref{sec:experiments}.

Before presenting our heuristic, we first introduce an important trade-off that is fundamental to federated learning and liken it to a similar trade-off in general SGD to better understand the impact of $m$.
To examine the trade-off, we ask the following question.
Given finite training time, which is better: aggregating many, but less informative, gradient updates at a higher rate or aggregating fewer, but more informative, ones at a lower rate?
In other words, is it better to make quick low-quality steps, or slow high-quality steps?
In standard centralized SGD, this trade-off is controlled by the size of the mini-batches $B$ used during each training round in which larger batch sizes will result in lower variance gradient estimates, but take longer to compute while smaller batch sizes will result in the opposite.
The choice of $B$, thus, directly affects per round computation time, the variance/quality of the gradient estimates, and the generalization of the final model \cite{bottou2010large,lin2018don}.
Unfortunately, in terms of wall-clock time versus test accuracy, $B$'s effect on final performance is mostly not understood, especially due to its effect on generalization.
% "The convergence speed of stochastic gradient descent is in fact limited by the noisy approximation of the true gradient."
%"the number of examples n effectively processed by the optimization algorithm"
% "Approximate optimization can achieve better expected risk because more training examples can be processed during the allowed time. The specifics depend on the computational properties of the chosen optimization algorithm."
% The above quotes from Bottou justify my approach/reasoning 
% Although even if GD is perfectly parallizable, SGD is still preferred due to generalization. communication has an outsized impact in FL

Moving on to FL, the same trade-off is also present, but is controlled by more than just batch size.
Now, the amount of data processed in each iteration is dictated by which devices are selected to participate in each round in addition to $B$.
Essentially, device scheduling can be recast as a dynamic batch size and data sampling problem for SGD where we will ignore the effect of having multiple local rounds $I$ for the time being.
In FL and distributed SGD, the wall-clock time versus final model accuracy trade-off is further complicated by introducing communication overhead to each round.
Part of the original question can be posed as is it better to schedule fewer devices per round such that collecting the updates takes less time, but ultimately provides a higher variance gradient estimate?
Or, is it better to schedule many devices per round? % where each iteration takes longer, but contains lower variance gradient estimates?
Again, the answer to this question is mathematically difficult to analyze and is dependent on the specifics of the given scenario and communication environment.
%While the present paper focuses on optimizing the communication portion of FL, it should be noted that if computation is the main bottleneck, then optimizing communication may see little gain in overall performance (see Amdahl's Law).

Since uniform sampling with replacement is more amenable to analysis, we choose this selection policy in order to illustrate the idea behind our heuristic.
We will ignore the hypothesized effect $m$ has on generalization of the final model \cite{keskar2016large} and will instead focus on a simplified problem.
How do we maximize the amount of data that is used to train the FL model in a given amount of time?
More specifically, we characterize the time it takes to learn per sample and then minimize this metric over $m$ to speed up convergence in terms of wall-clock time. % we will calculate the time it takes to go through one epoch of the complete dataset that is distributed over the $N$ nodes and then choose the $m$ that minimizes this.
The total time per aggregation round consists of both communication time and computation time, denoted as $\tau^\text{comm}_n$ and $\tau^\text{comp}$, respectively.
For simplicity, we will assume that every device has the same $\tau^\text{comp}$ and that computation occurs in parallel with all devices finishing simultaneously.
With computation determined, we now determine the expected time to communicate the parameters per round.
The expected time per sample can be expressed as
\begin{align}
    \Expectbracket{\frac{\tau^\text{comp} + \sum_{n=1}^N \Identity_n \tau^\text{comm}_n}{B I \, \sum_{n=1}^N \Identity_n}}
\end{align}

\begin{theorem}\label{thm:time_per_sample}
    Given Rayleigh fading and number of draws $m$, the expected time per sample is
    \begin{align}\label{eqn:time_per_sample}
        &\Expectbracket{\frac{\tau^\text{comp} + \sum_{n=1}^N \Identity_n \tau^\text{comm}_n}{B I \, \sum_{n=1}^N \Identity_n}} \nonumber \\
        & \qquad\qquad\qquad= \text{\jake{[will update if we keep section]}}
    \end{align}
\end{theorem}
\begin{proof}
    The proof can be found in Appendix \ref{sec:appendix3}.
\end{proof}

\begin{comment}

While our algorithm is agnostic to the distribution of the channel gain, in this section, we assume Rayleigh block fading.
Therefore, $|h_n|^2$ is exponentially distributed with parameter $\lambda_n=\frac{1}{\bar{\gamma}_n}$ where $\bar{\gamma}_n = \frac{2\sigma_n^2 P_\text{unif}}{N_0}$ is the average SNR for each device $n$, $\sigma_n^2$ is the Rayleigh fading parameter, and $P_\text{unif}$ is the transmit power used by all devices.
In order to satisfy the average time average power constraint, we set $P_n^t=P_\text{unif}\triangleq\min\{\Pmax, \bar{P}_n \cdot \frac{1}{q_n^t}\}=\min\{\Pmax, \bar{P}_n \cdot \frac{1}{1-(1-1/N)^{m}}\}$ since $\omega_n^t=\frac{1}{N}$ for all devices in uniform sampling.
The expected transmission time per device is then
\begin{align}
    \Expectbracket{\tau^\text{comm}_n} = \int_{0}^\infty \frac{\ell}{B\log_2\left( 1+\gamma \right)} \frac{1}{\bar{\gamma}_n} \exp\left(-\frac{\gamma}{\bar{\gamma}_n}\right) d\gamma
\end{align}
which does not converge.
In order to mitigate this, we assume that there is a minimum SNR $\gamma_\text{min}$ such that realizations less than $\gamma_\text{min}$ saturate to that value.
We now have,
\begin{align}
    \Expectbracket{\tau^\text{comm}_n} &= \int_{0}^{\gamma_\text{min}} \frac{\ell}{B\log_2\left( 1+\gamma_\text{min} \right)} \frac{1}{\bar{\gamma}_n} \exp\left(-\frac{\gamma}{\bar{\gamma}_n}\right) d\gamma + \int_{\gamma_\text{min}}^\infty \frac{\ell}{B\log_2\left( 1+\gamma \right)} \frac{1}{\bar{\gamma}_n} \exp\left(-\frac{\gamma}{\bar{\gamma}_n}\right) d\gamma \nonumber \\
    %&=\frac{\ell}{B\log_2\left( 1+\gamma_\text{min} \right)} \frac{1}{\bar{\gamma}_n}\int_{0}^{\gamma_\text{min}}  \exp\left(-\frac{\gamma}{\bar{\gamma}_n}\right) d\gamma + \frac{\ell}{B\bar{\gamma}_n}\int_{\gamma_\text{min}}^\infty \frac{1}{\log_2\left( 1+\gamma \right)} \exp\left(-\frac{\gamma}{\bar{\gamma}_n}\right) d\gamma \nonumber \\
    &=\frac{\ell\left(1-\exp\left(-\frac{\gamma_\text{min}}{\bar{\gamma}_n}\right)\right)}{B\log_2\left( 1+\gamma_\text{min} \right)}  + \frac{\ell}{B\bar{\gamma}_n}\int_{\gamma_\text{min}}^\infty \frac{1}{\log_2\left( 1+\gamma \right)} \exp\left(-\frac{\gamma}{\bar{\gamma}_n}\right) d\gamma,
\end{align}
for each device $n$.
Unfortunately, the second term does not have a closed-form expression, so we will have to use numerical integration to compute  $\Expectbracket{\tau^\text{comm}_n}$.

Since we consider TDMA and parallel computation, the total transmission time for one round is simply the computation time plus the sum communication time of the participating devices.
So, for a given $m$, the expected total training time is
\begin{align}
    \Expectbracket{\tau^\text{total}(m)} &= \Expectbracket{\tau^\text{comp} + \sum_{n=1}^N \Identity_n \tau^\text{comm}_n} \nonumber \\
    &=  \tau^\text{comp} + \left(1-\left(1-\frac{1}{N}\right)^{m}\right)\sum_{n=1}^N \Expectbracket{\tau^\text{comm}_n}.
\end{align}
Next, to get the time it takes to process an epoch of the total distributed dataset, we note that the expected number of samples seen in a given round is
\begin{align}
    \Expectbracket{B_\text{total}} &= B I \, \Expectbracket{\sum_{n=1}^N \Identity_n} \nonumber \\
    & = B I N \left(1-\left(1-\frac{1}{N}\right)^{m}\right)
\end{align}
where the final term is the expected amount of devices being selected in a given round, which is not simply $m$ due to replacement.
Finally, the expected time per epoch for a given $m$ is
\begin{align}\label{eqn:time_per_epoch}
    \Expectbracket{\tau^\text{epoch}(m)} = \frac{|\mathcal{X}|}{\Expectbracket{B_\text{total}}} \Expectbracket{\tau^\text{total}(m)}
\end{align}

With \eqref{eqn:time_per_epoch} in hand, we can choose the $m$ that minimizes the amount of time it takes for the model to learn from an epoch of the complete distributed dataset $\mathcal{X}$.
Since part of computing $\Expectbracket{\tau^\text{epoch}(m)}$ requires numerical integration, we simply iterate through values of $m$ and choose the one that minimizes the expression.
    
\end{comment}

\begin{figure}
    \centering
    \includegraphics[width=0.49\linewidth]{figures/optimal_m.png}
    \caption{Optimal number of draws for different computation times.}
    \label{fig:opt_m}
\end{figure}

In Figure \ref{fig:opt_m}, we plot \eqref{eqn:time_per_sample} for different computation times $\tau^\text{comp}$ and values for $m$.
The results show a clear optimal number of draws depending on the computation time.
As computation time increases, it is better to sample more devices as to take advantage of the parallel training that occurs as communicating those additional devices has lesser comparative impact on total round time.
We explore this empirically in the next section and find the same trends, though not the same optimal values for $m$.
